Cleaning Inconsistent Data in Temporal DL-Lite Under Best Repair Semantics

In this paper, we address the problem of handling inconsistent data in Temporal Description Logic (TDL) knowledge bases. Considering the data part of the Knowledge Base as the source of inconsistency over time, we propose an ABox repair approach. This is the first work handling the repair in TDL Knowledge bases. To do so, our goal is twofold: 1) detect temporal inconsistencies and 2) propose a data temporal reparation. For the inconsistency detection, we propose a reduction approach from TDL to DL which allows to provide a tight NP-complete upper bound for TDL concept satisfiability and to use highly optimised DL reasoners that can bring precise explanation (the set of inconsistent data assertions). Thereafter, from the obtained explanation, we propose a method for automatically computing the best repair in the temporal setting based on the allowed rigid predicates and the time order of assertions.

==> evaluation.tex <==
\section{Evaluation}
\label{sec-eval}

%\input{experiments1.tex}
%Ana : I started drafting some intro here...

%Due to the lack of \tdllitefpx ontologies available for testing and evaluating
% the translation
Since
% OWL cannot express \TDLLite ontologies,
there are no \TDLLite ontologies available for testing, in our
evaluation, we generated test ontologies synthetically, by extending
methods applied
%for testing the implementation
%of an automata
in the context of propositional temporal logic~\cite{Daniele1999ImprovedAG}.
We describe the test method in Subsection~\ref{subsec:test} and
our results in Subsection~\ref{subsec:results}.
%applied the test method
 
%To test the translation, we follow

%In this section, we discuss the implementation and the evaluation of results to show the effectiveness of the proposed %framework for inconsistency detection, 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Test Method}\label{subsec:test}

We extend the test method proposed by Daniele, Giunchiglia, and
Vardi~\cite{Daniele1999ImprovedAG} in the context of propositional
temporal logic to our case.  We analyse basic properties of the
translation of \TDLLite TBoxes into propositional temporal logic
formulas.  Following the mentioned method, we present two kinds of
analyses.
%
\begin{itemize}
\item \textbf{Average-behaviour}: For a fixed number of $N$ concept
  names and of $N$ role names, a fixed maximum \MaxQ for the value $q$
  in basic concepts of the form $ \geq q R$, a fixed number
  \lengthTbox of CIs in a TBox, and for increasing values
  \lengthConcept of the length of concept expressions in the TBox, we
  create batches $B(F,N,\lengthTbox,\lengthConcept,\MaxQ)$ of $F$
  random TBoxes. We can then plot the results against \lengthConcept
  and repeat the process for different values of $N$, \MaxQ, and
  \lengthTbox.
  %
\item \textbf{Temporal-behaviour}: For a fixed set of parameters
  $N, \MaxQ, \lengthTbox, \lengthConcept$, and for increasing values
  of the probability $P_t$ of generating the temporal operators
  $\{\D_P, \D_F, \B_P, \B_F\}$\footnote{For the temporal-behaviour, we focused on $\D_{P/F}$ and $\B_{P/F}$
  (and not in $\Next_{P/F}$) to analyse the behaviour several steps ahead of the current time point (as in~\cite{Daniele1999ImprovedAG}). } %\nb{A: what about $\Next$?}
  and the
  probability $P_g$ of generating global roles, we create batches
  $B(F,N,\lengthTbox,\lengthConcept,\MaxQ,P_t,P_g)$ of $F$ random
  TBoxes. We can then plot the results against $P_t$ and $P_g$ and
  repeat the process for different values of $N$, \MaxQ,
  \lengthConcept, and \lengthTbox.
% For a fixed  number 
% of $N$ concept names and of $N$ role names, a fixed maximun \MaxQ
% for the value $q$ in basic concepts of the form $ \geq q R$,
%  a fixed number \lengthTbox of CIs in a TBox,
%  a fixed size \lengthConcept of concept expressions in a TBox,
%  and for increasing values of  the probability $P_t$ of
%  generating the temporal operators $\{\D_P, \D_F, \B_P, \B_F\}$
% and  the probability $P_g$ of
%  generating global roles,
% %respectively,
%  we create batches  $B(F,N,\lengthTbox,\lengthConcept,\MaxQ,P_t,P_g)$
% of $F$ random TBoxes. We can then plot  the results against $P_t$ and $P_g$ and  %\lengthConcept.
% repeat the process %can be repeated
% for different
% values of $N$, \MaxQ, \lengthConcept, and \lengthTbox.
\end{itemize}

We now describe the procedure for generating random \TDLLite TBoxes
drawn uniformly from the space of \TDLLite TBoxes with \lengthTbox CIs
and concept expressions with length \lengthConcept (exactly
\lengthTbox and \lengthConcept, not up to \lengthTbox and
\lengthConcept). These concept expressions are formulated with concept
and role names in $\{A_1,\ldots,A_N\}$ and $\{R_1,\ldots,R_N\}$,
respectively, and $q\leq\MaxQ$ in basic concepts of the form
$ \geq q R$.  Since there is no risk of confusion, in what follows we
omit ``uniformly''.
%

For the average-behaviour analysis, we proceed as follows.  A random
concept expression with length one is generated by randomly choosing a
basic concept. Random concept expressions of length two are of the
form ${\sf op}(C)$ where $C$ is a random concept expression with
length one and ${\sf op}$ is randomly chosen from
$U=\{\neg, \Next_F,\Next_P, \Diamond_F, \Diamond_P,\Box_F, \Box_P\}$.
For concept expressions with length $L$ larger than one, ${\sf op}$ is
randomly chosen from $U\cup\{\sqcap\}$.  If ${\sf op}\in U$ (that is,
${\sf op}$ is unary) then the random concept expression is
${\sf op} (C)$, where $C$ is a random concept expression with length
$L-1$.  Otherwise, we randomly choose $K$ in $\{1, \ldots, L-2\}$ and
the random concept expression is $C\sqcap D$, where $C$, $D$ are
random concept expressions with length $K$ and $L-K-1$, respectively.
%
For the temporal-behaviour analysis we use the parameter $P_t$ to
increase the chance of generating the temporal operators in
$\{ \Diamond_F, \Diamond_P,\Box_F, \Box_P\}$ and the parameter $P_r$
increase the chance of generating a global role.  Random concept
expressions with length one are generated as for the average-behaviour
analysis.  For concept expressions with length two, the concept
expression is of the form ${\sf op}(C)$, where the probability that
${\sf op}=\Diamond_F$ is $\frac{P_t}{4}$ (same for ${\sf op}$ being
$\Diamond_P,\Box_F$ or $ \Box_P$) and the probability that
${\sf op}=\neg$ is $\frac{1-P_t}{3}$ (same for the other two unary
operators).  For concept expressions with length greater than two,
${\sf op}$ is again chosen from $U\cup\{\sqcap\}$ but now we
have %$\frac{P_t}{4}$ and
$\frac{1-P_t}{4}$ for the probability that ${\sf op}$ is $\neg$ (same
for $\Next_F,\Next_P,\sqcap$).
%~ the concept expression is of the form ${\sf op}(C)$ or $C\sqcap D$,
%~ where the probability that ${\sf op}=\Diamond_F$ is $\frac{P_t}{4}$
%~ (same for ${\sf op}$ being $\Diamond_P,\Box_F$ or $ \Box_P$)
%~ and the probability that ${\sf op}=\neg$ or ${\sf op}=\sqcap$
We have also generated ABoxes randomly, using the concept and role names
occurring in TBoxes.
%In particular, 

We are interested in investigating how different logical constructs
of \TDLLite TBoxes affect the size of the translation, the time for
computing the translation, and the time for deciding satisfiability 
using tools designed for LTL. % solvers and model checker.
%using different tools designed for solving this problem
%in LTL. In particular, 
In the temporal-behaviour analysis, we want to study
%(1)
how the presence of temporal operators
$\Diamond_F, \Diamond_P,\Box_F, \Box_P$ and global roles affect the
size of the translation and the time to compute the translation and to
check for satisfiability.

%\nb{Ana: on going...}

%Since we focus on the temporal aspects, the various  \tdllitefpx Tboxes, are generated randomnly, under conditions similar to %those used for the temporal-behavior analysis in ~\cite{Daniele1999ImprovedAG} for generating and testing temporal %propositional formulas.
%~ According to definition of a \tdllitefpx Tbox described in section~\ref{sec-tdl}. There are six parameters that defined a Tbox: 
%~ \begin{itemize}
%~ \item \lengthTbox : size of the set of CIs.
%~ \item $N$: size of the set of Concepts.
%~ \item \lengthConcept : length of each concept.
%~ \item \MaxQ : max cardinality for the quantified roles.
%~ \item $P_T$ : probability of generating temporal concepts.
%~ \item $P_R$ : probability of generating rigid roles.
%~ \end{itemize}
%~ For a given \lengthTbox , $N$, \lengthConcept , and for increasing values $P_T$ of the probability of generating Temporal Concepts with the temporal operators:$\{\Next_F, \Next_F, \D_P, \D_F, \B_P, \B_F\}$, an instance of a \tdllitefpx Tbox is produced randomly and given in input to the test procedure. After the satisfiability computation, a statistical analysis is performed and the results are plotted against $P_T$. The process can be repeated for different values of \lengthTbox , $N$ and \lengthConcept .

%~ Algorithm ~\ref{alg: tbox} proceeds by iteratively building a \tdllitefpx Tbox. The function \textproc{GenerateTbox} return  randomly a conjunction of \lengthTbox Concept Inclusion CIs or its negation with a probability $0,5$. From now on, unless otherwise specified, randomly called fonctions stands for randomly chosen with uniform distribution.The concepts occuring at the left and the right hand side of a CI, are created by calling the function  \textproc{GenerateConcept} defined in Algorithm~\ref{alg: concept} . 

%~ \begin{algorithm}
    %~ \caption{Generate a \tdllitefpx Tbox which is a set of Concept Inclusion CI}
    %~ \label{alg: tbox}
%~ \textbf{Inputs: <\lengthTbox , $N$, \lengthConcept ,\MaxQ , $P_T$,  $P_R$>}

%~ \textbf{Output:} \tdllitefpx Tbox   
    
%~ \begin{algorithmic}[h]
      
%~ \Function{GenerateTbox}{\lengthTbox,\lengthConcept, $N$,\MaxQ} 
       %~ \State  $Op = randomNegation()$ \tcp*[h]{$\neg \phi$}
       
        %~ \If{$L_{tbox}= 1$}
        %~ { 
        %~ \State ${C_1} = GenerateConcept()$
         %~ \State ${C_2} = GenerateConcept();$ 
         %~ \State {$tbox = {C_1} \sqsubseteq {C_2}$ \tcp*[h]{$C1\sqsubseteq C2$}}
         %~ \Return $Op ~tbox$
        %~ }
        %~ \Else
        %~ \Return $Op ~[GenerateTbox(L_{tbox}-1,L_c,N,Q_{max})\land GenerateTbox(1,L_c,N,Q_{max})]$ \tcp*[h]{$\phi \land \psi$}
	     
%~ \EndFunction  
%~ \end{algorithmic}   
%~ \end{algorithm}
%~ Algorithm~\ref{alg: concept} creates the set of $N$ random concepts of length exactly \lengthConcept. Each concept, according to its length, can be a Basic concept, a quantified role, a negated concept, a temporal concept or a conjunction of two concepts.

%~ \begin{algorithm}
%~ \caption{Generate  a set of Concepts}
%~ \label{alg: concept}
%~ \begin{algorithmic}[h]
%~ \Function{GenerateConcept}{{\lengthConcept, $N$, \MaxQ}} \Comment{Where n - size of the Concepts set}

  %~ \State $concept = GenerateBasicConcept(N, Q_{max})$\tcp*[h]{$A \mid \geq qR$} 		
  		
  		%~ \If{$L_{c} = 1$}
        %~ \Return $concept$
         
        %~ \ElseIf{$L_{c} = 2$}
        %~ {
          %~ \State {$Op = randomUnaryOp();$\Comment{unary operators: $\neg, \star=\{\Next,\Box, \Diamond$\}}
           %~ \Return $Op ~concept$  \tcp*[h]{$\neg C\mid \star C$}}
	    %~ }    
 	    %~ \Else
 	    %~ {
         %~ \State{ $Op = randomUnaryOrBinaryOp();$\Comment{Operators are: $\land$ and the Unary one's}}
         
         	%~ \If {$Op$ is unary}
         	%~ {
            %~ \State $concept = GenerateConcept(L_{c}-1,N,Q_{max});$
            %~ \Return $Op ~concept$
            %~ }
            %~ \Else{
            %~ \State $x= random[1,L_{c}-2];$
            %~ \State ${concept_1} = GenerateConcept(x,N,Q_{max});$
            %~ \State ${concept_2} = GenerateConcept(L_{c}-x-1,N,Q_{max});$
            %~ \Return $concept_1 \sqcap concept_2;$ \tcp*[h]{$C_1 \sqcap C_2$}           }
        %~ }         
%~ \EndFunction 
%~ \end{algorithmic}
%~ \end{algorithm}
%~ A unit-length random concept is a basic concept created by calling the function \textproc{GenerateBasicConcept} in Algorithm~\ref{alg: basic}. A random concept of length 2 is generated by generating $Op ~concept$, where $Op$ is a unary operator: $\{\neg, \Next,\Box, \Diamond\}$ chosen randomly with a probability $ \frac{P_T}{3}$ of chosing a temporal operators: $\Next,\Box,$or $\Diamond$ .
%~ Otherwise, with probability $ \frac{1-P_T}{2}$  of choosing either $\neg$ , or $\land$ , the operator $Op$ is randomly chosen. If $Op$ is unary, the random concept of length \lengthConcept is generated as $Op ~concept$, for some random concept  of length $\lengthConcept-1$. Otherwise, if $Op$ is binary, for some randomly chosen $1 \le x \le \lengthConcept-2$, two random concepts ${concept_1}$ and ${concept_2}$ of length $x$ and $\lengthConcept -x-1$ are produced, and the random concept $concept_1 \sqcap concept_2$  of \lengthConcept is generated. Since the set of operators we use is $\{\neg,\land, \Next,\Box, \Diamond\}$, random concepts for the temporal-behavior analysis are generated by setting $ P_T> \frac{3}{5}$ . \textcolor{red}{To check the value of Pt}. 


   %~ \begin{algorithm}
   %~ \caption{Generate  a set of Basic Concepts}
     %~ \label{alg: basic}
  %~ \begin{algorithmic}[h]
 %~ \Function{GenerateBasicConcept}{${N, Q_{max}}$}
        %~ \State $i = random[1,N]:$
        %~ \State $x_1 = randomBottomOrConceptNameOrQRole();$	
         
         %~ \If {$x_1$ is Bottom}
  		%~ {
  		    %~ \Return $ \bot $
  		 %~ }
  		%~ \ElseIf {$x_1$ is ConceptName}
  		%~ {
  		    %~ \Return $A_i$ \tcp*[h]{$A$}
  		 %~ }
  		   %~ \Else
  		%~ {
  		 %~ \State $x_2 = randomRigidOrFlexibleRole();$
          %~ \State $q = random[1,Q_{max}]:$ \Comment{q- cardinality of the role }	
          
          %~ \If {$x_2$ is RigidRole}
  		%~ {
  		    %~ \Return $qG_i$ \Comment{$G$- a rigid role}
  		 %~ }
  		   %~ \Else
  		%~ {         
          %~ \Return $qL_i$ \Comment{$L$- is a flexible role}
          %~ }
          %~ }
 %~ \EndFunction
 %~ \end{algorithmic}
 %~ \end{algorithm}
%~ The same, Algorithm~\ref{alg: basic} create a basic concept by randomly choosing, according to a uniform distribution, either one variable $A_i$ as a concept name, or one variable $qG_i$ as a quantified rigid role or a $qL_i$ as a quantified flexible role. In order to check  the impact of the use of roles in the complexity of the satisfiability calculation, we run tests for different caradinality values \MaxQ, and different values of  $P_R$ which is the probability of generating rigid roles then felexible one's.

%~ \begin{figure}[h]
  %~ \renewcommand{\arraystretch}{0}
  %~ \setlength{\fboxsep}{0mm}
  %~ \setlength{\tabcolsep}{0pt}
  %~ \begin{center}
    %~ \settowidth{\gapw}{bTD}%
    %~ \begin{tabular}[t]{@{}ll@{\quad}l@{}}
      %~ & \multicolumn{1}{c}{SAT } 
      %~ & \multicolumn{1}{c}{UNSAT }\\[1ex]
      %~ \begin{tabular}{lL}
        %~ \input{Adult-Labels.heat.tex}
      %~ \end{tabular}
      %~ &
        %~ \begin{tabular}{l*{10}{L}}
          %~ \input{Adult-Sat.heat.tex}
        %~ \end{tabular}
      %~ &
        %~ \begin{tabular}{l*{10}{L}}
          %~ \input{Adult-Unsat.heat.tex}
        %~ \end{tabular}\\
    %~ \end{tabular}\vspace*{-1.5em}
    
  %~ \end{center}
  %~ \caption[Heat map for Adult]{%
  %~ Heat map with the runtimes of Example~\ref{ex:1}.
    %~ Each rectangle represents the runtime in CPU seconds of
    %~ SAT and UNSAT KBs
    %~ %an
    %~ %ABox Assertion
    %~ with different sizes %for different size either SAT or UNSAT
    %~ on LTL solvers.
    %~ The runtimes are given in colours as follows:\\
   % Heat map of the runtimes on Adult example.
   % Each rectangle represents the runtime in CPU seconds of an
   % Abox Assertion for different size either SAT or UNSAT with LTL solver
   % with runtimes given in colours as follows:\\
    %~ {\scalebox{0.77}{%
%~ \setlength{\fboxsep}{0mm}% box size
%~ \begin{tabular}{@{}*{13}{N@{\ }l@{\ }}@{}}
       %~ 0 & $<\lmt{0.01}$ sec &
       %~ 1 & $>\lmt{0.01}$ sec, $\leq\lmt{0.25}$ sec &
       %~ 2 & $>\lmt{0.25}$ sec, $\leq\lmt{0.50}$ sec &
       %~ 3 & $>\lmt{0.50}$ sec, $\leq\lmt{1}$ sec
             %~ \\
       %~ 4 & $>\lmt{1}$ sec, $\leq\lmt{2}$ sec &
       %~ 5 & $>\lmt{2}$ sec, $\leq\lmt{4}$ sec &
       %~ 6 & $>\lmt{4}$ sec, $\leq\lmt{8}$ sec &
       %~ 7 & $>\lmt{8}$ sec, $\leq\lmt{16}$ sec 
                                        %~ \\
       %~ 8 & $>\lmt{16}$ sec, $\leq\lmt{32}$ sec &
       %~ 9 & $>\lmt{32}$ sec, $\leq\lmt{64}$ sec &
      %~ 10 & $>\lmt{64}$ sec, $\leq\lmt{125}$ sec &
      %~ 11 & $>\lmt{125}$ sec, $\leq\lmt{250}$ sec 
            %~ \\
      %~ 12 & $>\lmt{250}$ sec, $\leq\lmt{500}$ sec &
      %~ 13 & $>\lmt{500}$ sec, $\leq\lmt{1000}$ sec &
      %~ 14 & T/O, OoM or Fail
      %~ \end{tabular}
    %~ }}}\label{Adult-Heat}
%~ \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Methodology and Materials}
\subsection{Experimental environment and \LTL solvers}
%\nb{to be checked and enhanced}

We briefly present the hardware/software environment where the tests
have been performed together with the off-the-shelf \LTL solvers used.

\paragraph{\bf Hardware and Software.} We run the experiments 
 % in sequence
on a server with 8 Genuine Intel 3.6 GHz processors, and 4 GB memory
running Debian GNU/Linux 10 (buster) with 64 bit kernel 4.19.0-8.  Run
time and memory usage were measured with
runlim\footnote{\url{http://fmv.jku.at/runlim/}}.

% \paragraph{\bf Hardware and Software} We run the experiments on a server built with 7 Genuine Intel 3.6 GHz processors, and 4 GB memory running Debian GNU/Linux 10 (buster) with 64 bit kernel 4.19.0-8. 
% We measured run time and memory usage with runlim\footnote{\url{http://fmv.jku.at/runlim/}}.

%\paragraph{\bf Set-up}

We set the run time to a timeout of 600 CPU seconds, while memory is set up to 1 GB.
% memory space.
In the test, we denote with `T/O' the case where the solver either
runs out of memory or it times out. With `Fail' we denote the case
where the solver encountered an unexpected error condition.
% the time
% value if the \LTL solver is not able
% to determine the satisfiability of the formula within that time or
% memory space and
%
% the `Fail' value if LTL solver encountered some other
% error condition and stopped before the timeout or memory space were
% reached.

\paragraph{\bf \LTL Solvers.} We considered various \LTL solvers
adopting different reasoning strategies:
% from these classes of approaches:
\emph{reduction to model checking}, \emph{tableau-based algorithms},
and \emph{temporal resolution}. The chosen solvers have been already
considered in the literature to test their performances for checking \LTL
formula satisfiability~\cite{SchuppanD11,DBLP:conf/cade/HustadtOD17}.
% in evaluations of solvers for
% satisfiability of LTL and in related works about particular tools
%
As for the solvers based on model checking, we opted for
\texttt{NuXMV} %\nb{A: changed to NuXMV as suggested by Marco}
using the following options: BDDs (Binary Decision Diagrams), SAT
(based\nb{A: changed} on SAT techniques and also denoted as BMC for
Bounded Model Checking), and the variant IC3 (known also as
\emph{Property Directed
  Reachability})~\cite{nusmv:Cimatti02,nuxmv:CavadaCDGMMMRT14,ic3}.
% Moreover, we also considered
% \texttt{nuXmv} with the variant IC3 (known also as \emph{Property
%   Directed Reachability}) \cite{nuxmv:CavadaCDGMMMRT14}.
BDD is a complete satisfiability technique but it requires space
exponential in the number of variables, and it is also sensitive to
the variable order. On the other hand, BMC reduces the problem to SAT
by testing the formula for satisfiability in models with length
bounded by a fixed\nb{A: added} $k$, % of size at most $k$,
%and thus
giving sound but incomplete results. %\nb{AO: to check}
% Lastly, nuXmv has been built on NuSMV so that they offers the same
% behaviour for both BDD and BMC methods. However, although
% IC3 follows an incremental approach, this novel algorithm
IC3 computes approximations of reachability in a backward-search
fashion.

The solver \texttt{pltl}~\cite{pltl:98} implements a tableau-based
algorithms. We run \texttt{pltl} with the options \texttt{graph} and
\texttt{tree}. %The \texttt{tree} method builds a rooted tree with ancestor cycles and passes up information about unfulfilled eventualities. The graph method also builds a rooted tree in a depth first left to right manner, but allows cross branch edges, from\nb{A: not at all  clear to me} one branch to a previous branch, as well as ancestor cycles (see also~\cite{pltl:graph}).  
Both methods build rooted trees with ancestor cycles but different search strategies (see also~\cite{pltl:graph} for details).  
Compared with the traditional
tableau-based translation, Aalta (Another Algorithm for LTL To Büchi
Automata) \cite{Aalta:19}, implements a new algorithm by introducing
the concept of \emph{Obligation Set} for LTL formulas. Aalta
integrates two functions: LTL-to-Büchi translation and LTL
satisfiability checking.
 %
Finally, \texttt{TRP++UC}~\cite{trpuc:Schuppan13} implements temporal
resolution, and has been used with the option dfs/bfs (Depth-First
search/Breadth-First search).
% to choose dfs/bfs in loop search.
%In particular,
This solver has been built on %the previous
\texttt{TRP++} \cite{TRP:HustadtK03}. Despite the aim of \texttt{TRP++UC} is to extract
unsatisfiable cores for \LTL, we used the legacy features
of \texttt{TRP++} by running the solver with the unsatisfiable cores
option disabled.

%%%%%%%%%%%%%%%%%
\subsection{Results}
\label{subsec:results}

In what follows we evaluate the efficiency and the scalability of our
tool using two evaluation tests of increasing difficulties.
The first test is based on the \textbf{toy scenarios} described in
Examples~\ref{ex:1} and~\ref{ex:2}. The second test
applies the test method for \textbf{generating TBoxes randomly}, as described in Subsection~\ref{subsec:test}. 
Our benchmark is available from \url{http://crowd.fi.uncoma.edu.ar/temporalDLLite/benchmark/}.
%, which includes 6195 instances, 
%~ \begin{itemize}
 %~ \item Test on toy examples
 %~ \item Test on synthetic TBoxes
%~ \end{itemize}
%
%\paragraph{\bf Limitations of Solvers}
We discovered in our experimental evaluation that \texttt{Aalta} presents limitations when the \LTL input has more than 1200 propositional variables. %The solver is not able to process such inputs.

%In particular, for each test we check the satisfiability using model
%checkers: \NuSMVBDD, \NuSMVSBMC, \NuXMVBDD and \NuXMVSBMC and LTL
%solvers: \Aalta, \PLTLGraph, \PLTLTree, \TRPppBFS, and \TRPppDFS and
%we measured the reasoning time under a timeout of 6000 CPU seconds and
%1 GB memory space. We indicate the `T/O' value if the LTL solver is
%not able to determine the satisfiability of the formula within that
%time or memory space and the `Fail' value if LTL solver encountered
%some other error condition and stopped before the timeout or memory
%space were reached.

\input{5.1-toyexampletest}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> implementation.tex <==
%~ \begin{figure}[tp]
 %~ \centering
 %~ \includegraphics[width=\textwidth]{diagram-2.pdf}
 %~ \caption{Tool Architecture}
 %~ \label{fig:framework}
%~ \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}
\label{sec-impl}

In this section, we describe the main components of our
implementation. We first present the transformation framework, where
\TDLLite\ KBs are mapped to \LTL\ formulas, and then we describe the
graphical web tool for generating $\mathcal{ER_{VT}}$ temporal
diagrams (see~\cite{AKRZ:ER10} for details on mapping
$\mathcal{ER_{VT}}$ to a \TDLLite\ TBox, we discuss this more in
Subsection~\ref{sec:wb}).
%
The suite of tools involved in this framework is composed by a core
Java library, a visual tool for $\mathcal{ER_{VT}}$ diagrams and an
API to connect them. All of the tools are open source and are
available at
\url{https://bitbucket.org/gilia/workspace/projects/TCROW}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Transformation Framework}

Here we comment on our framework.  As shown in
Figure~\ref{fig:framework}, by using our suite of tools one can reason
over \TDLLite\ KBs. We consider two forms of input.  In the first one,
the user draws a temporal conceptual schema using the
$\mathcal{ER_{VT}}$ modelling language which is then automatically
mapped into a \TDLLite TBox.  The graphical interface also allows users to insert temporal data, which is mapped into an ABox.  In the
second, the tool receives as input a \TDLLite KB directly within the
Java code.  Since\nb{A: changed} the OWL language does not support the temporal
dimension, we have created % these two
ad-hoc methods for % representing
capturing \TDLLite
KBs % in practice
in the tool.  As mentioned in the Introduction, the tool contains
an implementation of the translation of \TDLLite\ KBs into \LTL\
formulas (Section~\ref{sec-translation}).  This allows the use of
off-the-shelf \LTL\ solvers to perform satisfiability checks for
\TDLLite\ KBs.  The translation is a process with (at most) five main
stages:
% 
\begin{enumerate}
%~(1)~
\item Translate the input $\mathcal{ER_{VT}}$ temporal diagram into
  a \TDLLite\ TBox;
%~(2)
\item Mapping the resulting TBox (with the possible addition of ABox
  assertions) into a \QTLO formula (as in Section~\ref{QTL-reduction});
%~(3)
\item Remove the past operators (see Section~\ref{Future-reduction});
\item Obtain the \LTL\ translation via the grounding
  (see Section~\ref{PTL-reduction}); and
%~(4)~
\item Adapt\nb{A: delete ``rewrite'' as suggested by REV2} the
  resulting \LTL formula according to the syntax of the corresponding
  solver.
\end{enumerate}
% \nb{AO: talk about the step of \PTL to \LTL already here? (This is
% the paragraph about the figure since there step appears there..)}
%in case the \QTLO formula
%derives from a $\TDLLiteN$ TBox, then we map it directly to $\LTL$ by
%performing the grounding described in
%Section~\ref{PTL-reduction};

\begin{figure}[t]
 \centering
 \begin{tikzpicture}[scale=0.8, transform shape]
%~ \begin{overpic}[scale=0.75]{Framework2.pdf}
     %~ \put(1,1){\includegraphics[scale=0.21]{er.pdf}}  
  %~ \end{overpic}
   every node/.style={anchor=south west,inner sep=0pt},
        x=1mm, y=1mm,
      ]   
     \node (fig1) at (0,0)
       {\includegraphics[scale=0.6]{Framework2.pdf}};
     \node (fig2) at (-4.7,1.7)
       {\includegraphics[scale=0.33]{er.pdf}};  
%    \draw (0, 0) node[inner sep=0] {\includegraphics[width=\textwidth]{Framework2.pdf}};
    \draw (-3.1, -1.9) node {\small{\TDLLite}}; %{\tiny{\tdllitefpx}};
%    \node[above=0 of image] {Hello world};
 \draw (-5.4, -2.5) node {\small{\TDLLite}};
   % \draw (0, 0) node[above=0 of image] {\includegraphics[width=\textwidth]{er.pdf}};
    \draw (-0.7, -1.9) node {\small{\QTLO}};
   \draw (1.5, -1.9) node {
\begin{tabular}{ c }
        Remove \\
        past
\end{tabular}        };
%        \draw (1.5, -1.9) node {No past};
    \draw (3.7, -1.9) node {$LTL$};
    %\draw (0.5,2.77) node {ABox};
\draw (0.5,1.6) node {\begin{tabular}{ |l| c| r| }
\hline
Person & Status & Time\\
\hline
\hline
  %John & Minor & 1 \\
  John & Minor & 1 \\
  John & Adult & 2 \\
    John & Minor & 3 \\
\hline
\end{tabular}};
\end{tikzpicture}
  \caption{Translation Steps}
 \label{fig:framework}
\end{figure}

There are two shortcuts for this process
(see~Figure~\ref{fig:framework}).  The first is when the \TDLLite\ KB
is encoded directly within the Java code.  The second is when the
ontology does not contain past operators, i.e., it is expressed is the
\TDLLiteN logic.  While\nb{A: small changes} for clarity of
presentation, Section~\ref{Future-reduction} describes the removal of
past modalities as a translation from \PTL to \LTL, in the current
implementation we remove past operators already from the \QTLO
encoding and then grounding the resulting formula, still obtaining an
equisatisfiable \LTL translation.\nb{A: commented next sentence}
% The translation in Section~\ref{Future-reduction} was
% described in the propositional case for presentation purposes, it can
% be easily adapted to the \QTLO language.

%\nb{on going}

% Before giving the obtained LTL formula to a solver, we need to consider if solvers are able to deal with both past and future temporal operators or only with future operators. In this sense, many of the %state-of-the-art %AO: better avoid because other solvers such as LS4 were not included, 
% solvers in the literature %considered for this work
% such as Aalta \cite{Aalta:19}, pltl \cite{pltl:98} and TRP++UC \cite{trpuc:Schuppan13} handle only future operators, while only NuSMV/nuXmv model checker \cite{nusmv:Cimatti02,nuxmv:CavadaCDGMMMRT14} handle both kind of operators. \nb{AO: explain that this is over naturals}

%We also consider the case in which the ontology does not have past operators
%and therefore does not need 

%~ We notice that the step~(3.2) adds an additional burden to our
%~ process aiming at reducing \QTLO formulas to \QTLO pure-future
%~ formulas. In particular,
%~ as will be clear from the experiments, the
%~ size of the resulting formula will substantially increase in the
%~ number of \LTL atoms.

% , as
% described in sub-section~\ref{Future-reduction}. As a consequence, it
% is possible to proceed into two directions: sending the resulting LTL
% formulae (including past operators) to the NuSMV/nuXmv model checker
% or giving the equi-satisfiable LTL pure future formulae to some of the
% SAT solvers or even the same NuSMV/nuXmv.


% From the implementation point of view, the framework is structured in modules clearly defined in order to delegate responsabilities to each one. In particular, the first module encodes a starting  $\mathcal{ER_{VT}}$ model into a \tdllitefpx KB following the semantics given in \cite{}. Once the \tdllitefpx KB has been generated, it is given as input to the next module, which is in charge of converting the KB into a set \QTLO axioms. Finally, as the  $\mathcal{ER_{VT}}$ semantics is given in terms of irreflexive temporal operators and the solvers work with reflexive ones, the framework addresses this mismatch at this point by making strict the \QTLO formulae, i.e putting $\Next_F$ and $\Next_P$ in front of each $\Box_F, \Diamond_F$ and $\Box_P, \Diamond_P$,respectively. At the moment when the processing is split in two branches, the \QTLO formula is grounded as a LTL formulae and is ready to be checked if both past and future are considered. On the contrary, the \QTLO formula is then reduced to an equi-satisfiable \QTLO future formulae before being grounded as a LTL one. Complementary functionalities of this reasoner implements the last step of this pipeline, which aiming at rewriting the resulting LTL formula using the syntax of the corresponing solver. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The $\mathcal{ER_{VT}}$ Web Tool}
\label{sec:wb} 

Involving knowledge engineers, domain experts and end-users in the
construction, maintenance, and use of conceptual models requires a
strong interaction between them. The use of common languages along
with appropriate methodologies is a way to effectively manage such
interactions and to successfully guide the whole process.  However,
methodologies for conceptual modelling appear to be fragmented across
several tools and workarounds \cite{VigoBJS14}, and visualisation
methods proposed are weakly integrated to logic-based reasoning
tools~\cite{DBLP:conf/jowo/BraunCF19}.

Based on these motivations, we have developed an open source graphical
tool for designing $\mathcal{ER_{VT}}$ temporal
diagrams~\cite{DBLP:conf/er/ArtaleF99,artale:franconi:john09,AKRZ:ER10}, named
{\tt
  crowd-$\mathcal{ER_{VT}}$}\footnote{\url{http://crowd.fi.uncoma.edu.ar/ervt-gui/erd_editor.php}}
and based on the architecture presented in~\cite{Braun-KI}.  The idea
behinds the tool is: (i) to define a suitable abstraction level for
temporal modelling tasks involving both users and the underlying
methodologies of conceptual data modelling; and (ii) to understand better how %and to what extent
logic-based knowledge representation systems can be integrated with
visual languages in a tool.

\begin{figure}[t]
\centering
	\begin{minipage}[b]{0.55\linewidth}
		\centering
		\includegraphics[width=\textwidth]{ervt-example.png}
		\caption{$\mathcal{ER_{VT}}$ graphical interface}
		\label{fig:figure1}
	\end{minipage}
\hspace{0.2cm}
	\begin{minipage}[b]{0.35\linewidth}
		\centering
		\includegraphics[width=\textwidth]{ervt-example-data.png}
		\caption{Widget to add temporal  data}
		\label{fig:figure2}
	\end{minipage}
\end{figure}

{\tt crowd-$\mathcal{ER_{VT}}$} supports temporal conceptual modelling
in $\mathcal{ER_{VT}}$ providing a visual environment, a comprehensive
set of $\mathcal{ER_{VT}}$ primitives, and an interface to
off-the-shelf reasoners as depicted in Figure~\ref{fig:framework}.
Moreover, the tool provides an interface to add temporal data
assertions (i.e., a temporal ABox) to populate the $\mathcal{ER_{VT}}$
model. Once both the $\mathcal{ER_{VT}}$ diagram and the temporal data
have been specified, they are jointly sent to the server, where they
are ultimately translated into \LTL.  When the reasoning process ends,
the tool provides a link where the user can download the intermediate
translations, including the \TDLLite\ TBox and ABox encodings, the
respective \QTLO translations, the encoding where past operators have
been removed (if any), the final $\LTL$ formula, and the output of a reasoner.

To show how the tool works, we revisit the running examples introduced
in Section~\ref{ex:1} showing the corresponding $\mathcal{ER_{VT}}$
diagram, and the temporal data assertions.  Figures~\ref{fig:figure1}
and~\ref{fig:figure2} show the graphical interface extending
Examples~\ref{ex:1}-\ref{ex:2}. In addition to the entities {\sf
  Person}, {\sf Adult} and {\sf Minor}, and the
attribute\footnote{\emph{Attributes} in CMs associate an entity to a
  concrete value and are usually encoded as roles in the corresponding
  DL TBox encoding.}\nb{A: added footnote} {\sf Name}, the tool allows to specify \emph{visual marks}
for each temporal primitive in $\mathcal{ER_{VT}}$. For example, {\sf
  Person} is set as a \emph{global} entity (using the {\sc S} mark,
standing for \emph{Snapshot} following the temporal ER
notation~\cite{AKRZ:ER10} for global entities), while each {\sf Minor}
will become an {\sf Adult} sometime in the future (expressed by the
dotted line labeled \texttt{DEV}, standing for Dynamic EVolution). The
axiom stating that minors and adults are disjoint is modelled as a
disjoint composed ISA (the {\bf d} labeled circle). The fact that
every adult stays always adult in the future is captured by the dotted
line labeled \texttt{PEX} (standing for Persistence).
% primitive \texttt{PEX}, respectively.
In Figure~\ref{fig:figure2}, we show the user interface to specify temporal
assertions, showing the person {\sf John} and his name at different
timestamps.
% Finally, to check the consistency of a set of temporal
% data for this example, the tool enables an interface to assert the
% status of the person John and his name at different timestamps.

The set of visual primitives also includes binary relationships (both
\emph{global} and \emph{local} relationships are supported), and
cardinalities are limited to the
$1..1$ and $0..N$ cases.
% over such relationships.
Cardinalities on attributes are limited to just $1..1$. Entities and
attributes can be also tagged as \emph{global} or \emph{local}. Lastly,
other forms of temporal operators between entities are also supported: \texttt{TEX} (standing for Transition EXtension) and
\texttt{DEX$^{-}$} (standing for Dynamic EXtension) (see~\cite{DBLP:conf/er/ArtaleF99,artale:franconi:john09,AKRZ:ER10}).

% Lastly, \texttt{TEX}, i.e. transition extension, and
% \texttt{DEV$^{-}$}, i.e. dynamic extension, as introduced in the
% formalisation of $\mathcal{ER_{VT}}$ can be added to models by drag
% and dropping a target entity over another one, which is the origin of
% that constraint.
 

%encoding of these diagrams into DL, validating of  ontologies by interacting with off-the-shelf reasoners, and  visual feedback about model consistency and implicit properties. Moreover, the tool allows to integrate diverse namespaces and supports OWL 2 and OWLlink \cite{conicet:Liebig_owllink:dig} standards. 

%we are not aware of any prover supporting past operators. For that an additional step is performed before the $\LTL$ translation to reduce \QTLO formulas to \QTLO future formulas as described in sub-section~\ref{Future-reduction}.   
  
%%%%%%%%%%%%%%%





\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> toyexampletest.tex <==
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Toy Scenarios Experiment.}
\label{test:toy examples}
We report here on the experimental results conducted by pairing the
TBoxes of the toy examples, as reported in Section~\ref{sec:intro},
with different ABoxes which may yield satisfiable (SAT) and
unsatisfiable (UNSAT) KBs.  The sizes of the ABoxes vary from $20$ to
$50$ assertions (distributed over different time points).  The number
of propositional variables in the resulting \LTL formula starts from a
minimum of 14 variables, for the KB as in Example~\ref{ex:1}\nb{A:
  added}, and ranges from 180 to 2336 variables for
Example~\ref{ex:2}\nb{A: added} depending on the increasing sizes of
the tested ABoxes.  The experimental results for the cases where the
TBox is as in Examples~\ref{ex:1} and~\ref{ex:2} are shown in
Figures~\ref{Adult-Heat} and \ref{Name-Heat}, respectively.  For\nb{A:
  chenged} the
UNSAT cases, we explicitly inserted 
inconsistent assertions % at each time point
(e.g., {\sf John} being both {\sf Minor} and {\sf
  Adult}, % {\sf Minor}...
in case of Example~\ref{ex:1}, while we added more than 1 name to the
same person in case of Example~\ref{ex:2}).
%We visualize results in Table~\ref{Adult-FullF} in Figure~\ref{Adult-Heat}
The results, presented in the form of `heat maps', represent\nb{A:
  changed} the runtime of the KB satisfiability checking for
increasing ABox sizes (in columns) and different solvers (in lines).
% in the columns, the runtime of the KB satisfiability checking with
% each different ABox distinguishing the results tested \LTL solvers.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \renewcommand{\arraystretch}{0}
  \setlength{\fboxsep}{0mm}
  \setlength{\tabcolsep}{0pt}
  \begin{center}
    \settowidth{\gapw}{bTD}%
    \begin{tabular}[t]{@{}ll@{\quad}l@{}}
      & \multicolumn{1}{c}{SAT } 
      & \multicolumn{1}{c}{UNSAT }\\[1ex]
      \begin{tabular}{lL}
        \input{Adult-Labels.heat.tex}
      \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Adult-Sat.heat.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Adult-Unsat.heat.tex}
        \end{tabular}\\
    \end{tabular}\vspace*{-1.5em}    
  \end{center}
  \caption[Heat map for example1]{%
    Heat map with the runtimes for Example~\ref{ex:1}.
    Each rectangle represents the runtime in CPU seconds of
    SAT and UNSAT KBs % with different sizes
    % on LTL solvers.
    with ABoxes of increasing size.
    The runtimes are given in colours as follows:\\
    {\scalebox{0.77}{%
\setlength{\fboxsep}{0mm}% box size
\begin{tabular}{@{}*{13}{N@{\ }l@{\ }}@{}}
       0 & $<\lmt{0.01}$ sec &
       1 & $>\lmt{0.01}$ sec, $\leq\lmt{0.25}$ sec &
       2 & $>\lmt{0.25}$ sec, $\leq\lmt{0.50}$ sec &
       3 & $>\lmt{0.50}$ sec, $\leq\lmt{1}$ sec
             \\
       4 & $>\lmt{1}$ sec, $\leq\lmt{2}$ sec &
       5 & $>\lmt{2}$ sec, $\leq\lmt{4}$ sec &
       6 & $>\lmt{4}$ sec, $\leq\lmt{8}$ sec &
       7 & $>\lmt{8}$ sec, $\leq\lmt{16}$ sec 
                                        \\
       8 & $>\lmt{16}$ sec, $\leq\lmt{32}$ sec &
       9 & $>\lmt{32}$ sec, $\leq\lmt{64}$ sec &
      10 & $>\lmt{64}$ sec, $\leq\lmt{125}$ sec &
      11 & $>\lmt{125}$ sec, $\leq\lmt{250}$ sec 
            \\
      12 & $>\lmt{250}$ sec, $\leq\lmt{500}$ sec &
      13 & $>\lmt{500}$ sec, $\leq\lmt{1000}$ sec &
      14 & T/O, OoM or Fail
      \end{tabular}
    }}}\label{Adult-Heat}
\end{figure}%
%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \renewcommand{\arraystretch}{0}
  \setlength{\fboxsep}{0mm}
  \setlength{\tabcolsep}{0pt}
  \begin{center}
    \settowidth{\gapw}{bTD}%
    \begin{tabular}[t]{@{}ll@{\quad}l@{}}
      & \multicolumn{1}{c}{SAT }
      & \multicolumn{1}{c}{UNSAT } \\[1ex]
      \begin{tabular}{lL}
        \input{Name-Labels.heat.tex}
      \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Name-Sat.heat.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Name-Unsat.heat.tex}
        \end{tabular}\\   
    \end{tabular}\vspace*{-1.5em}
  \end{center}
  \caption[Heat map for Name]{%
  Heat map with the runtimes of Example~\ref{ex:2}.
  Each rectangle represents the runtime in CPU seconds of
  SAT and UNSAT KBs  with ABoxes of increasing size
    (the colours are as in the previous figure).\\
    {\scalebox{0.77}{%
        \setlength{\fboxsep}{0mm}% box size
      }}}\label{Name-Heat}
\end{figure}
%%%%%%%%%%%%%%%%

Solvers\nb{A: various changes in this paragraph} had better
performances over SAT instances compared to UNSAT ones, except \TRPpp
which fails to scale even to small ABoxes.  Moreover,
\texttt{NuXMV-SBMC} fails regardless the size of the model in UNSAT
cases (also when running in the simpler scenario of
Example~\ref{ex:1}).
% In Example~\ref{ex:1}, no model was found by \texttt{NuXMV-SBMC} (with
% and without translation)\nb{A: remove} at size 20.
Considering the experimental setting of Example~\ref{ex:1}
(Fig.~\ref{Adult-Heat}), we note that the best performers over UNSAT
cases were \texttt{NuXMV} with BDD and \texttt{NuXMV} with
IC3, \texttt{Aalta} and \texttt{pltl}.
% Moreover, \texttt{NuXMV-SBMC} fail regardless the size of the model in
% UNSAT cases.
% Unlike the first experiment, the results obtained from
% the second
The more involved setting of Example~\ref{ex:2} clearly shows that the
BMC option is the best for the SAT cases while \texttt{NuXMV} with the
IC3 option stands out in the UNSAT case.
%Important point to note is that
\texttt{Aalta} performs well but only when the \LTL input does not exceed
$1200$ variables.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \renewcommand{\arraystretch}{0}
  \setlength{\fboxsep}{0mm}
  \setlength{\tabcolsep}{0pt}
  \begin{center}
    \settowidth{\gapw}{bTD}%
    \begin{tabular}[t]{@{}llllll@{\quad}l@{}}
       & \multicolumn{1}{c}\texttt{1 concept}
      & \multicolumn{1}{c}\texttt{3 concepts}
      & \multicolumn{1}{c}\texttt{5 concepts}\\  
      \begin{tabular}{lL}
        \input{1average-Labels.heat.tex}
      \end{tabular}
      &
        \begin{tabular}{l*{10}{L}}
          \input{1average-Sat.heat1.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{1average-Sat.heat2.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{1average-Sat.heat3.tex}
        \end{tabular}
    &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Labels.heatRight.tex}
        \end{tabular}
           \end{tabular}\vspace*{-1.5em}
  \end{center}
  \caption[Heat map for average behaviour]{%
    Heat map of the runtimes on randomly generated TBoxes according to
    the average behaviour (the colors are as in the toy experiments).}
  \label{average-Heat}
\end{figure}
%
\begin{figure}[t]
  \renewcommand{\arraystretch}{0}
  \setlength{\fboxsep}{0mm}
  \setlength{\tabcolsep}{0pt}
  \begin{center}
    \settowidth{\gapw}{bTD}%
    \begin{tabular}[t]{@{}llllll@{\quad}l@{}}
       & \multicolumn{1}{c}\texttt{1 concept}
      & \multicolumn{1}{c}\texttt{3 concepts}
      & \multicolumn{1}{c}\texttt{5 concepts}\\  
      \begin{tabular}{lL}
        \input{Temporal-Labels.heat.tex}
      \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Temporal-Sat.heat1.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Temporal-Sat.heat2.tex}
        \end{tabular}
      &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Temporal-Sat.heat3.tex}
        \end{tabular}
        &
        \begin{tabular}{l*{4}{L!{\color{white}\vline}}}
          \input{Labels.heatRight.tex}
        \end{tabular}
    \end{tabular}\vspace*{-1.5em}
  \end{center}
  \caption[Heat map for the temporal behaviour]{%
    Heat map of the runtimes on randomly generated TBoxes according to the temporal behaviour (the colors are as in the toy experiments).\\
    {\scalebox{0.77}{%
        \setlength{\fboxsep}{0mm}% box size
      }}}\label{Temporal-Heat}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Randomly Generated TBoxes.}
\label{test:synthetic TBoxes}
%
With this experiment setting we investigate the reasoning scalability
over randomly generated TBoxes (see Section~\ref{subsec:test}). These
are KBs with an empty ABox and with (mostly) SAT TBoxes.  In this is
evaluation we only consider \LTL solvers that performed well in the
previous toy scenarios, namely, \texttt{NuXMV-SBMC}, \texttt{Aalta},
and \texttt{NuXMV-IC3}. Again, we use `heat maps' to illustrate the
obained results. For each solver,\nb{A: added} the results are
reported in two consecutive lines: the first line denoting the case where
$\lengthConcept = 5$, while the second has $\lengthConcept =
10$. Each square represents the runtime for different values of $N$
according to the following legenda:
%
\begin{itemize}
\item For the average behaviour, TBoxes were generated with the
  parameters $F = 20$, $N = 1,3,5$, $\lengthTbox = 5,10,15,20$
  (columns), $\lengthConcept = 5,10$ (lines), and $\MaxQ = 5$.
  %
\item For the temporal behaviour, TBoxes are generated with the
  parameters $F = 20$, $N = 1,3,5$, $\lengthTbox = 10$,
  $\lengthConcept = 5,10$ (lines), $\MaxQ = 5$, $P_t =0.1,0.9$, and
  $P_g =0.7,0.9 $ (the first two columns are with $P_g=0.7$ and two
  values for $P_t=0.1, 0.9$, the last two columns are with $P_g=0.9$
  and again $P_t=0.1, 0.9$).
\end{itemize}

\nb{G: paragraph added.} Concerning the number of propositional variables in the resulting \LTL formulae and the current experimental setting, 
the average behaviour generated formulae from 400 and up to 8400 variables (\lengthConcept = 5), and
from 500 and up to 14500 variables (\lengthConcept = 10). On the other hand, the
temporal behaviour generated from 400 and up to 3500 variables (\lengthConcept = 5), and
from 950 and up to 6600 variables (\lengthConcept = 10).


Due \nb{A: new sentence} to the increase in the number of variables
when removing the past operators, as expected solvers perform better
on TBoxes expressed with only future operators (i.e., on $\TDLLiteN$
TBoxes) as shown on lines 3, 4 and 5 on both Figures~\ref{average-Heat}
and~\ref{Temporal-Heat}, with the BMC option performing better than
IC3.
%
% We can see that solvers perform well on TBoxes expressed with
% only future operators as shown on lines 3, 4 and 5 of the two Heat
% maps in Figures~\ref{average-Heat} and \ref{Temporal-Heat}.
%
In the general case (presence of both past and future
operators),\nb{A: small changes} the \LTL translation that removes
past operators at the cost of a linear increase of the propositional
variables % to the corresponding \LTL formula which
makes the reasoning more difficult.  Moreover, there is not much
difference between the heat map corresponding to the average
behavior (Fig.~\ref{average-Heat}) and the one of the temporal
behavior (Fig.~\ref{Temporal-Heat}). In our experimental
setting, this indicates that the \LTL solvers were more affected by
the number of propositional variables involved in the formula than by
the number of temporal operators in the formula. Once again the BMC
option is the best one for reasoning on SAT cases.
%~ \subsubsection{TBoxes Randomly Generated}
%~ \label{test:synthetic TBoxes}
%~ With this last experiment our objective is to focus on the reasoning scalability over randomly generated  TBoxes
%~ (Subsection~\ref{subsec:test}). In this is evaluation we only consider LTL solvers that performed well in the previous experiments: \texttt{NuSMV-BMC}, \texttt{Aalta}, \texttt{NuXMV-IC3}. And we compare them on 2400 synthetic TBoxes. The result is shown in Figure~\ref{average-Heat}. For the average behaviour, TBoxes are generated, for F=100, N=1,3,5, \lengthTbox =5,10,15,20,\lengthConcept =5,10 and \MaxQ =5. For the temporal behaviour, TBoxes are generated, for F=100, N=1,3,5, \lengthTbox =5,10,15,20,\lengthConcept =5,10 and \MaxQ =5.
%~ The results shows the runtime for each value of N and each solver. we can clearly see that solvers performs well on Tboxes expressed with only futur operators, otherwise their translation to future add more propositional  variables to the corresponding LTL formula which would make the reasonning more difficult such as Aalta. 
%~ Once again we notice that the BMC option is the best for reasonning on SAT cases.
% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

